From Mathematical Reasoning to Code: Generalization of Process Reward Models in Test-Time Scaling

Recent advancements in improving the reasoning capabilities of Large Language Models have underscored the efficacy of Process Reward Models (PRMs) in addressing intermediate errors through structured feedback mechanisms. This study analyzes PRMs from multiple perspectives, including training methodologies, scalability, and generalization capabilities. We investigate the interplay between pre-training and reward model training FLOPs to assess their influence on PRM efficiency and accuracy in complex reasoning tasks. Our analysis reveals a pattern of diminishing returns in performance with increasing PRM scale, highlighting the importance of balancing model size and computational cost. Furthermore, the diversity of training datasets significantly impacts PRM performance, emphasizing the importance of diverse data to enhance both accuracy and efficiency. We further examine test-time scaling strategies, identifying Monte Carlo Tree Search as the most effective method when computational resources are abundant, while Best-of-N Sampling serves as a practical alternative under resource-limited conditions. Notably, our findings indicate that PRMs trained on mathematical datasets exhibit performance comparable to those tailored for code generation, suggesting robust cross-domain generalization. Employing a gradient-based metric, we observe that PRMs exhibit a preference for selecting responses with similar underlying patterns, further informing their optimization.

==> 05_related_work.tex <==
\section{Related Work}
Process Reward Models have emerged as a promising approach to improve these capabilities by providing granular feedback on intermediate steps during solution generation. Recent studies \cite{zhang2025lessons,lightman2023lets} have identified challenges related to data annotation and evaluation methods, leading to solutions like consensus filtering mechanisms to enhance performance.

Further research has introduced heuristic algorithms and model adaptations to advance LLMs' reasoning abilities. Ma \cite{ma2024learning} developed a heuristic greedy search algorithm that surpasses traditional techniques on mathematical benchmarks, while Zhang \cite{zhang2024entropy} introduced an entropy-regularized PRM leveraging KL-regularized Markov Decision Processes for significant improvements on key benchmarks. %Lightman et al. demonstrated the superiority of process supervision over outcome supervision, highlighting the benefits of active learning in solving complex problems.

Automated models like Math-Shepherd \cite{wang2024math} have been developed to minimize manual annotations, showing notable improvements in LLM performance. Setlur et al. \cite{setlur2024rewarding} introduced Process Advantage Verifiers (PAVs), optimizing reasoning steps and increasing efficiency in reinforcement learning, further emphasizing the role of PRMs in  mathematical reasoning.

Test-time scaling strategies have also been crucial in optimizing LLM performance. Efficient allocation of test-time compute, as illustrated by Setlur et al. \cite{setlur2024rewarding}, can significantly outperform larger models. Chen \cite{chen2024simple} proposed a two-stage algorithm that reduces failure rates exponentially with increased compute, while Zhang \cite{zhang2024scaling} found that model scaling offers greater benefits than data scaling. Yue \cite{yue2024inference} highlighted performance gains through optimal inference scaling.

Research into scaling laws in reinforcement learning and reward modeling has identified consistent power-law relationships. Gao \cite{gao2023scaling} explored distinctions between optimization methods, and Neumann \cite{neumann2024alphazero} noted scaling effects in multi-agent RL. Rafailov \cite{rafailov2024scaling} and Hilton \cite{hilton2023scaling} examined overoptimization and intrinsic performance, respectively, illustrating the importance of understanding scaling laws for AI alignment and model design.

This paper builds on these foundational studies to explore the scalability and generalization of PRMs, aiming to optimize their performance across diverse reasoning tasks and enhance the overall capabilities of LLMs.

% \textbf{Process Reward Models}
% Recent research on Process Reward Models (PRMs) for mathematical reasoning in Large Language Models (LLMs) has revealed several key insights. Zhang et al. (2025) identified challenges in data annotation and evaluation methodologies, proposing a consensus filtering mechanism to improve model performance. Ma et al. (2023) demonstrated the effectiveness of PRMs during inference, developing a heuristic greedy search algorithm that outperformed Chain of Thought on mathematical benchmarks. Zhang et al. (2024) introduced an entropy-regularized PRM, achieving improvements on MATH and GSM8K benchmarks through KL-regularized Markov Decision Processes. Lightman et al. (2023) found that process supervision significantly outperforms outcome supervision on the MATH dataset, with their model solving 78\% of problems from a representative subset. They also showed that active learning enhances process supervision's efficacy. These studies collectively highlight the potential of PRMs in improving LLMs' mathematical reasoning capabilities and provide valuable insights for future research in process supervision models.

% Recent research has focused on developing Process Reward Models (PRMs) to improve mathematical reasoning in Large Language Models (LLMs). PRMs provide step-by-step feedback on reasoning processes, potentially outperforming outcome-based supervision (Lightman et al., 2023; Zhang et al., 2025). Challenges in PRM development include data annotation and evaluation methodologies, with human annotation and LLM-as-judge approaches showing better performance than Monte Carlo estimation (Zhang et al., 2025). Wang et al. (2023) introduced Math-Shepherd, an automated PRM that eliminates the need for manual annotations and demonstrates significant improvements in LLM performance on math tasks. Setlur et al. (2024) proposed Process Advantage Verifiers (PAVs), which measure progress at each reasoning step, leading to more efficient exploration during search and reinforcement learning. These advancements in PRMs have shown promising results in enhancing LLMs' mathematical reasoning capabilities, with improvements in accuracy and compute efficiency compared to traditional outcome-based methods.

% The Lessons of Developing Process Reward Models in Mathematical Reasoning, 

% Rewarding Progress: Scaling Automated Process Verifiers for LLM Reasoning

% Math-Shepherd: Verify and Reinforce LLMs Step-by-step without Human Annotations

% let's verify step by step.

% \textbf{Test-Time Scaling}

% Recent research explores test-time scaling strategies for large language models (LLMs). Snell et al. (2024) demonstrate that optimally scaling test-time compute can outperform larger models, improving efficiency by over 4x compared to best-of-N baselines. Chen et al. (2024) propose a two-stage algorithm with provable scaling laws, showing exponential decay in failure probability as test-time compute increases. Zhang et al. (2024) investigate scaling effects in LLM finetuning, revealing power-based multiplicative joint scaling laws between finetuning data size and other factors. They find that LLM finetuning benefits more from model scaling than pretraining data scaling. In a different approach, Zhang et al. (2024) introduce LLMTTT, a test-time training method for graphs using LLMs as annotators, demonstrating significant performance improvements for out-of-distribution generalization. These studies collectively highlight the potential of test-time scaling and adaptation techniques to enhance LLM performance across various tasks.



% Recent research explores scaling test-time computation in large language models (LLMs) to improve performance. Snell et al. (2024) found that optimally allocating test-time compute can outperform larger models, while Chen et al. (2024) proposed a two-stage algorithm with provable scaling laws for test-time compute. Zhang et al. (2024) investigated scaling factors in LLM finetuning, revealing a power-based multiplicative joint scaling law between finetuning data size and other factors. Yue et al. (2024) focused on inference scaling for retrieval augmented generation (RAG), demonstrating nearly linear performance gains with optimal compute allocation. These studies highlight the importance of efficient test-time computation strategies, such as adaptive allocation (Snell et al., 2024), knockout tournaments (Chen et al., 2024), and in-context learning and iterative prompting for RAG (Yue et al., 2024). The findings suggest that optimizing test-time compute can significantly enhance LLM performance across various tasks and settings.

% Scaling LLM Test-Time Compute Optimally can be More Effective than Scaling Model ParametersCharlie S

% A Simple and Provable Scaling Law for the Test-Time Compute of Large Language Models

% When Scaling Meets LLM Finetuning: The Effect of Data, Model and Finetuning Method

% Inference Scaling for Long-Context Retrieval Augmented Generation



% \textbf{Scaling law for Reward Modeling}
% Recent research has explored scaling laws in reinforcement learning (RL) and reward modeling. Gao et al. (2022) investigated reward model overoptimization, finding that the relationship between proxy and gold reward models follows different functional forms depending on optimization method. Neumann  Gros (2022) observed power-law scaling of player strength with neural network parameters and compute in multi-agent RL. Rafailov et al. (2024) extended the study of overoptimization to Direct Alignment Algorithms, uncovering similar degradation patterns to classical RLHF at higher KL budgets. Hilton et al. (2023) introduced "intrinsic performance" to analyze scaling in single-agent RL, discovering power-law relationships between performance, model size, and environment interactions. Across these studies, consistent power-law scaling patterns emerged, with optimal model size scaling as a power law of the compute budget. These findings have implications for AI alignment, model design, and understanding the fundamental relationships between compute, model size, and performance in RL systems.

% Recent research has revealed power-law scaling relationships in various aspects of machine learning. In language models, performance scales as a power-law with model size, dataset size, and compute used for training (Kaplan et al., 2020). Similar scaling laws have been observed in reinforcement learning, where player strength in game-playing models like AlphaZero scales as a power law with neural network parameter count and compute (Neumann  Gros, 2022). For single-agent reinforcement learning, intrinsic performance scales as a power law with model size and environment interactions across different environments (Hilton et al., 2023). These scaling laws suggest that larger models are more sample-efficient and that optimal compute-efficient training involves using very large models with relatively modest amounts of data. However, in reinforcement learning from human feedback, optimizing too much against an imperfect reward model can hinder ground truth performance, following Goodhart's law (Gao et al., 2022).

